Snowmass2021 Cosmic Frontier White Paper: Observational Facilities to Study Dark Matter

We present an overview of future observational facilities that will significantly enhance our understanding of the fundamental nature of dark matter. These facilities span a range of observational techniques including optical/near-infrared imaging and spectroscopy, measurements of the cosmic microwave background, pulsar timing, 21-cm observations of neutral hydrogen at high redshift, and the measurement of gravitational waves. Such facilities are a critical component of a multi-pronged experimental program to uncover the nature of dark matter, while often providing complementary measurements of dark energy, neutrino physics, and inflation.

==> authors-old.tex <==
% Facilitators
\author[1]{Sukanya Chakrabarti}
\author[2]{Ting S. Li}
\author[3]{Neelima Sehgal}
\author[4]{Joshua D. Simon}

% Contributors
\author[5,6]{Simon Birrer}

\author[7]{Daniel Grin}
%\author[]{Ian Dell'Antonio}
\author[8,9,10]{Alex Drlica-Wagner}
\author[11]{Anze Slosar}
\author[12]{Yu-Dai Tsai}
\author[]{Duncan Brown}

% Affiliations
\affil[1]{School of Physics and Astronomy, Rochester Institute of Technology, 84 Lomb Memorial Drive, Rochester, NY 14623}
\affil[2]{Department of Astronomy and Astrophysics, University of Toronto, 50 St. George Street, Toronto ON, M5S 3H4, Canada}
\affil[3]{Physics and Astronomy Department, Stony Brook University, Stony Brook, NY 11794, USA}
\affil[4]{Observatories of the Carnegie Institution for Science, Pasadena, USA, 91101}
\affil[5]{Kavli Institute for Particle Astrophysics and Cosmology and Department of Physics, Stanford University, Stanford, CA 94305, USA}
\affil[6]{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}
\affil[7]{Department of Physics and Astronomy, Haverford College, 370 Lancaster Avenue, Haverford, Pennsylvania 19041, United States}
\affil[8]{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\affil[9]{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\affil[10]{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}
\affil[11]{Brookhaven National Laboratory, Upton NY 11973}
\affil[12]{Department of Physics and Astronomy, University of California, Irvine, CA 92697-4575, USA}
